Mitigating Pooling Bias in E-commerce Search via False Negative Estimation

Efficient and accurate product relevance assessment is critical for user experiences and business success. Training a proficient relevance assessment model requires high-quality query-product pairs, often obtained through negative sampling strategies. Unfortunately, current methods introduce pooling bias by mistakenly sampling false negatives, diminishing performance and business impact. To address this, we present Bias-mitigating Hard Negative Sampling (BHNS), a novel negative sampling strategy tailored to identify and adjust for false negatives, building upon our original False Negative Estimation algorithm. Our experiments in the Instacart search setting confirm BHNS as effective for practical e-commerce use. Furthermore, comparative analyses on public dataset showcase its domain-agnostic potential for diverse applications.

==> tex/background.tex <==
\section{Background}


The general relevance assessment task can be formulated as the following: Each training batch, denoted as $\mathcal{B}$, is composed of three distinct components: a set of queries $\mathcal{Q}$, a corresponding set of products $\mathcal{P}$, and associated relevance scores $\mathcal{R}$. Given a search query $q_i \in \mathcal{Q}$ and a product  $p_i\in \mathcal{P}$, the model is responsible for assessing the degree of relevance between $q_i$ and $p_i$, which is denoted by $r_i \in \mathcal{R}$. In this section, we briefly introduce the existing query-product relevance model at Instacart empowered by conventional negative sampling strategies and more effective cross encoder architecture in development, as the technical context of this work. 

\subsection{Search Embedding Model at Instacart}

Instacart has an effective and efficient embedding model to measure the relevance between queries and products, which is widely used in search retrieval, ranking, and many other surfaces \cite{xie2022embedding}. The search embedding model follows a typical bi-encoder design, where queries and products are passed through their corresponding encoders independently, denoted as $BE_{Q}$ and $BE_{P}$, and input query-product pair $(q_i, p_i)$ are transformed into dense embeddings as follows:

\begin{equation}
\begin{gathered}
    \mathbf{e}_i^q =\text{BE}_{Q}(q_{i}),\\
    \mathbf{e}_i^p =\text{BE}_{P}(p_{i}),
    \end{gathered}
\end{equation}

Relevance between a query and a product is computed via cosine similarity between their embeddings, i.e.:

\begin{equation}
\label{eq:sim}
    \hat{\mathbf{r}}_i = \text{sim}(\mathbf{e}_i^q, \mathbf{e}_i^p)
\end{equation}

During the training phase, similarity scores can be efficiently calculated through a series of matrix transpositions and multiplications, making the process computationally efficient. For the inference, the embeddings $\mathbf{e}_i^q$ and $\mathbf{e}_i^p$ can be pre-computed offline and cached. During inference, relevant products for an incoming search query are retrieved using the query's embedding via approximate nearest neighbor search (ANN), and the estimated relevance score $\hat{\mathbf{r}}_i$ is passed to the ranker service as a feature to determine the final ranking of $p_i$ for search term $q_i$. 

% The relevance score corresponding to the input pair, i.e., $\mathbf{r}_i$, serves as the prediction targeted, hence forms the loss along with $\mathbf{sim}_i$:

% \begin{equation}
%     \mathbf{L} = -\sum_i r_i \log(\text{sim}_i) + (1 - r_i) \log(1 - \text{sim}_i)
% \end{equation}


% \subsection{In Batch Negative Sampling}


% Regardless of model architecture, the query-product relevance model requires training data with positive (relevant) and negative (irrelevant) ($q_i$, $p_i$) pairs. 
While the supervised training of search embedding model benefits from supervised learning using ground-truth label $\mathcal{R}$, it also suffers from the insufficiency of negative cases. In e-Commerce search, positive ($q_i$, $p_i$) data can be obtained from past search logs with converted products quite easily. However, while these query-product pair serve as golden-standard positive cases, high-quality negative cases, which should have been able to help the model to acquire capability of distinguishing irrelevant products from relevant ones, are naturally absent. 


A straightforward solution is selecting products that do not result in search conversions as negative examples for a given query. Nevertheless, unconverted products may not necessarily be irrelevant to the search query, because users' decision can be swayed by many factors other than relevance such as price, size, visual presentation, personal preference for flavor or brand, etc. This is confirmed in our data verification process in examining search logs from Instacart, a leading e-commerce player in on-line grocery shopping, where we found more than 4\% of query-product pairs from the search logs with zero historical conversions are labeled as positive (relevant) by human annotators. 

A common alternative approach to address the lack of negative samples issue is in-batch negative sampling. Given query $q_i$ and in-batch products $p_j$, the vanilla sampling process can be formulated as follows:

\begin{equation}
\label{vanilla}
\begin{gathered}
    \mathbf{r}(q_i, p_j)=0 \ \ s.t. i \neq j, p_j \in \text{rand\_select}_{k}(\mathcal{P}).
\end{gathered}
\end{equation}

where $\text{r}(q_i, p_j)$ denotes the relevance between query $q_i$ and any in-batch products $p_j$, and $\text{rand\_select}_k$ represents the function that randomly selects $k$ distinct products within the batch. Unpaired query and product are assigned with the label 0 that indicates irrelevance.

Previous studies \cite{kalantidis2020hard, robinson2020contrastive} have claimed the usefulness of introducing hard negative samples during the sampling procedure due to their informativeness. Our present search embedding model allows us to obtain the representation of query and product, hence select products similar with the query as negative samples. The hard negative sampling process with the negative size equal to $k$ can be represented as follows:

\begin{equation}
\label{hard}
  \mathbf{r}(q_i, p_j)=0 \ \ s.t. j \in argmax_{k} (\text{sim}(\mathbf{e}_i^q, \mathbf{e}_j^p)).
\end{equation}


However, indiscriminately assuming irrelevance between a given query $q_i$ and in batch product $p_j$ will inevitably introduce false negatives. Our case study based on Instacart search log shows that for the query "\textit{Honey}", the product "\textit{Honey 100\%}", which is definitely relevant to the query but is not the product in this pair, will be retrieved as the top ranked hard negative sample by the hard negative sampler mentioned in Eq. \ref{hard}, clearly prove the existence of pooling bias. The pooling bias diminishes the quality of augmented negative pairs, impeding the model from conducting precise relevance assessment and necessitating a concrete solution. 

% To avoid the bias introduced during the sampling process, we propose the False Negative Estimation (\method) method. We will introduce this method in detail in the following section.


\subsection{Cross Encoder in E-commerce Search}

Previous work \cite{reimers2019sentence} has demonstrated the cross encoder as a more powerful solution to capture the relationship between two input sentences compared with the bi-encoder. The cross encoder, denoted as $\text{CE}$, takes the concatenation of query and product sentences as input, and directly outputs the relevance score after a series of transformations as follows:

\begin{equation}
    \hat{\mathbf{r}}_i = \text{CE}([q_i \cdot p_i])
\end{equation}
where $[\cdot]$ denotes the concatenation operation. 

% We adopt Cross Entropy as the loss to guide the training of $\mathbf{CE}$ as follows:

% $$\mathcal{L} = -\sum_i (\mathbf{r_i} \log(\hat{\mathbf{r}}_i) + (1 - \mathbf{r_i}) \log(1 - \hat{\mathbf{r}}_i))$$

% where $r_i \in \mathcal{R}$ is the ground truth relevance between $q_i$ and $p_i$.

The bi-encoder model encodes the query and the product separately; once the model is trained, the embedding for a given query is fixed regardless of which product it is paired with. In contrast, in cross encoder, the output of each intermediate layer is determined jointly by both query and product, which allows more interactions between the two and richer context to be extracted. 

However, the cross encoder does not output embedding of either query or product, thus presents two primary limitations: first, while training the cross encoder, similarity score calculation via matrix multiplication, as mentioned in Eq \ref{eq:sim}, is precluded due to the lack of corresponding embeddings. The score can only be obtained through aggregating queries and products in the input stage, proposing significant computational challenge. The problem becomes particularly severe when parameter $k$ in Eqs. \ref{vanilla} and \ref{hard} is large, constraining the scale of negative sampling; second, instead of simply computing the cosine similarity between the cached embeddings, cross encoder requires the full computation of a transformer model on the fly during inference time, which result in an $O(mn)$ computational complexity that can significantly increase the latency of the system. Given this limitation, in e-Commerce $\text{CE}$ is often adopted for re-ranking only while bi-encoders are retained for retrieval and first-stage ranking. In this work we follow this tradition and adopt $\text{CE}$ as part of a re-ranker for a small subset of top products pre-selected by the retrieval engine and first-stage ranking.

% second, the absence of dense embedding of query and product impedes the in-batch contrastive learning. In the ranking scenario, training samples are usually records taken from search history, naturally labeled as positive. Negative samples are mainly generated from in-batch sampling  





==> tex/conclusion.tex <==
\section{Conclusion}

In conclusion, we propose a novel method, referred to as {\method}, mitigating pooling bias by identifying potential false negative samples that arise during the training of a cross encoder for e-commerce retrieval. {\method} utilizes query similarity to estimate the likelihood that a sampled query-product pair is a false negative. To comprehensively address this issue, we have developed two modules, namely the pseudo label generator and sampling regularization, each designed to mitigate the pooling bias introduced by false negatives. By combining these two modules, we establish the {\modelfull}, denoted as {\model}. Through a series of experiments along with A/B testing conducted within the Instacart environment, we have demonstrated that {\model} significantly enhances the performance of the cross encoder. This enhancement holds considerable promise for its application in the e-commerce setting. Furthermore, the success of {\model} on the STS Benchmark dataset implies its applicability extends beyond the e-commerce domain.

% \xiaochen{Xiaochen: Main contents have been covered in this manuscript.\\ To do for polishment:\\}





% \xiaochen{1. Polish the graph demonstrating the whole architecture / sampler.\\}
% \xiaochen{2. Add a section about case study before/after using the sampler.\\}
% \xiaochen{3. Polish the writing.\\}
% \xiaochen{4. Provides details about deployment.\\}




==> tex/experiment.tex <==
\section{Experiment}

To demonstrate the efficacy of our proposed {\modelfull} strategy, we conduct experiments on both public and private datasets. Besides, we incorporate {\sampler} with Instacart search system to validate the practical value of {\modelfull} strategy. 


\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{fig/system.pdf}
\vspace{-0.1in}
\caption{Overview of Instacart's reranking system incorporated with \model-boosted cross encoder. \xiaochen{Polish this one tomorrow. The figure is available at \url{https://docs.google.com/presentation/d/1WFF1t6F0c5q1k8xtevENC5Lh1PRjGDg0HfTIY2RdXYY/edit?usp=sharing} for editing.}}
\label{fig:system}
\vspace{-0.1in}
\end{figure*}

% \subsection{False Negative Estimation}
% \label{sec:FNE}


% \subsection{False Negative Estimation}
% \label{sec:FNE}



\subsection{Semantic Textual Similarity}

To examine the effectiveness of \method, we first conduct our experiment on Semantic Textual Similarity (STS) task. In the STS task, the similarity between two pieces of text is expected to be predicted by a model, analogous to the general search use cases. 



\subsubsection{Dataset}
For the dataset, we adopt the commonly used STS Benchmark \footnote{http://ixa2.si.ehu.eus/stswiki/index.php/STSbenchmark} to simulate the search use case. 

\subsubsection{Implementation}

MiniLM-L3-v2 \footnote{https://huggingface.co/sentence-transformers/paraphrase-MiniLM-L3-v2} and MiniLM-L-2-v2 \footnote{https://huggingface.co/cross-encoder/ms-marco-MiniLM-L-2-v2} serve as bi-encoder and cross encoder in our experiments.
During the training, the bi-encoder is frozen.

% They share the same architectures with models in our production end, hence ensure the consistency with experiments in Section \ref{sec: offline_results}. 
% Similar with our experiments on Instacart in-house datasets, the bi-encoder is frozen during the training. 

% \xiaochen{Xiao: are the bi-encoder and the cross encoder finetuned on STS first?}

% \xiaochen{Xiaochen: No, the experiments are in the same setting. Thanks for proposing the concern and I've explicitly described this part.}

% \xiaochen{Taesik: Just wanted to understand, we used bi-encoder trained on Instacart data for hard negative estimation, and fine-tuned the cross encoder with the estimation from the bi-encoder for STS dataset?}

% \xiaochen{Xiaochen: Yes, your understanding is absolutely correct. The bi-encoder is frozen during the fine-tuning of cross encoder. Also, for your concerns of using a weak learner to guide the strong learner, it is found possible to use sentence transformer to guide LLM\cite{zhang2022automatic}, so I believe this issue is not problematic.}

% \xiaochen{Taesik: interesting to know that a bi-encoder trained on Instacart data helped improve the performance of the cross-encoder for STS. I imagine if we used a bi-encoder trained on STS, then I guess we would observe even more gains.}

% \xiaochen{Xiaochen: Actually, in the STS task, I just utilize a pretrained sentence transformer imported from huggingface, without any pretrianing on our own data. It is not pretrained on the STS task, but I believe it is not the focus of our research as current choice can still achieve performance boosting.}

% \xiaochen{Taesik: That totally makes sense.}

\subsubsection{Evaluation Metric}

As STS Benckmark evaluation dataset does not allow list-wise comparison, we decide to adopt the evaluation metrics utilized in script provided in the document of cross encoder \footnote{https://github.com/UKPLab/sentence-transformers/blob/master/examples/training/cross-encoder/training\_stsbenchmark.py}, which are Pearson correlation coefficient and Spearman correlation coefficient. Besides, we leverage Area under the ROC Curve (AUROC) as an additional evaluation metric for a more fair comparison. These three metrics perform pair-wise evaluation simultaneously. 

\subsubsection{Baselines}
We compare our proposed {\modelfull} ({\model}) with Vanilla Negative Sampling (VNS) and Hard Negative Sampling (HNS), they serves as natural baselines widely used in diverse scenario. Furthermore, we extend our experiment by adding the following advanced baselines specially designed for handling false negatives:

\begin{itemize}
\item \textbf{STAR} (\textbf{S}table \textbf{T}raining \textbf{A}lgorithm for
dense \textbf{R}etrieval) \cite{zhan2021optimizing} is a training pattern developed to combine random negative sampling with hard negative sampling to optimize the training process of bi-encoder. In this study, we transfer their strategy of performing combination to the case of cross encoder.
\item \textbf{FALSE} (\textbf{F}alse neg\textbf{A}tive samp\textbf{L}es aware contra\textbf{S}tive l\textbf{E}arning model) \cite{zhang2022false} is a strategy of detecting false negative samples in unsupervised contrastive learning scenario. We transfer this method to the supervised training of cross encoder by adopting their idea of capturing false negatives based on inter-sample similarity.
\item \textbf{CET} (\textbf{C}oupled \textbf{E}stimation \textbf{T}echnique) \cite{cai2022hard} leverages a subordinate cross encoder, i.e., observer,  to monitor and correct false negative bias during the training of the primary cross encoder, i.e. reranker. 
\end{itemize}

To perform fair comparison, we also choose MiniLM-L-2-v2 as cross encoder for baselines. For methods involving hard negative sampling, i.e., HNS and STAR, we adopt the bi-encoder same to BHNS (MiniLM-L3-v2) to guide the selection of hard negatives.

\begin{table}[]
\begin{tabular}{l|l|rrr}
\hline
                       &                                         & \multicolumn{1}{l}{Pearson} & \multicolumn{1}{l}{Spearman} & \multicolumn{1}{l}{AUROC} \\
                       \hline

\multirow{3}{*}{k = 2} & VNS                         & 67.61        & 77.05 & 90.18       \\
                       & HNS                     & 66.74                       & 74.57  & 89.24                    \\
                       & STAR \cite{zhan2021optimizing}                     & 59.95                       & 72.04  & 88.28                     \\
                       & FALSE \cite{zhang2022false}                         & 70.56        & 77.10 & 90.12       \\
                       & CET \cite{cai2022hard}                         & 75.87        & 75.21 & 88.96       \\
                      & \CC{}\model (ours) & \CC{}\textbf{78.32}                       & \CC{}\textbf{77.37} & \CC{}\textbf{90.64}                       \\
                       \hline
\multirow{3}{*}{k = 4} & VNS                         & 67.53                       & 76.67 &  89.99                    \\
                       & HNS                    & 67.09                       & 74.11 &  88.93                      \\
                       & STAR \cite{zhan2021optimizing}                      & 62.93                       & 72.30 &  88.52               \\
                       & FALSE \cite{zhang2022false}                         & 70.76        & 76.55 & 89.76       \\
                       & CET \cite{cai2022hard}                         & 75.78        &  75.12 & 88.91       \\
                        & \CC{}{\model}   (ours) &  \textbf{\CC{}77.97}                       & \CC{} \textbf{76.91} & \CC{} \textbf{90.34}                     \\
                       \hline
\multirow{3}{*}{k = 8} & VNS                         & 67.49        & 76.12 & 89.90       \\
                       & HNS                  & 71.76                       & 74.81 & 89.19                      \\
                       & STAR \cite{zhan2021optimizing}                      & 65.57                      & 73.01  & 88.56            \\
                       & FALSE \cite{zhang2022false}                         & 71.85        & 76.07 & 89.43       \\
                       & CET \cite{cai2022hard}                         & 76.53        & 75.45 & 89.07       \\
                       & \CC{}\model (ours) & \CC{}\textbf{77.30}                        & \CC{}\textbf{76.37} & \CC{}\textbf{90.05}      \\
                       \hline
\end{tabular}
\caption{Experiments on STS Benchmark Dataset. The highest score is shown in \textbf{boldface}.}
\label{STS}
\end{table}


\subsubsection{Result}
We test different sampling sizes to validate the superiority as well as the robustness of our proposed {\model}. The results are listed in Table ~\ref{STS}, where $k$ is the negative sampling size. Comparison across different sampling strategies implies that hard negative sampling may not contribute to decent performance due to the introduced false negative bias, while BHNS equipped with our proposed {\model} is enabled to handle the pooling bias, and thus perform better via the bias mitigation.

It is also worth noting that {\model} outperforms CET, which involves an additional cross encoders to observe and eliminate false negatives. It indicates that leveraging a frozen bi-encoder to simply estimate likelihood of false negatives is superior to supervised sophisticated approaches demanding extra training, showcasing the soundness of the hypothesis we propose in Section \ref{sec:FNE}, as well as validating the rationale behind our design. 

% Furthermore, compared with our experiments in the search setting provided in Section \ref{sec: offline_results}, the performance enhancement after leveraging {\model} is more considerable. The significance of improvement implied that there are more false negatives while applying negative sampling strategy in the STS task, since two arbitrary sentences are improbable to be absolutely irrelevant to each other, thus indiscriminately assuming the label between them as 0 is more problematic and significantly more harmful to the training process. 






\subsection{Offline Experiment}\label{instacart_exp}

\subsubsection{Dataset}

Datasets used for training and evaluating the cross encoder model come from Instacart's on-going data collection effort to benchmark search relevance, where a random sample of search queries and the products ranked in top display positions are sent for human annotation every month to judge the relevance between queries and products. The annotators categorize each (query, product) pair into five categories: 

\begin{itemize}
    \item \textbf{Strongly Relevant}: The product is exactly the type of product the search query is asking for.
    \item \textbf{Relevant}: The product fits the search query, but there are likely better alternatives.
    \item \textbf{Somewhat Relevant}: The product is not exactly what the search query asks for, but it is understandable why it shows up.
    \item \textbf{Not Relevant}: The product is not what the search query asks for and it is unclear why it shows up.
    \item \textbf{Offensive}: The product is unacceptable and creates a bad user experience.
\end{itemize}

To help the model grasp the finer granularity in relevance, we convert the above categories into soft labels in the training dataset by taking “Strongly Relevant” as 1, “Relevant” as 0.5, “Somewhat Relevant” as 0.2, and “Not Relevant/Offensive” as 0.1. Scores from multiple annotators for the same (query, product) pair are averaged. 

Annotated classes in the evaluation dataset are converted with a coarser stroke, with "Strongly Relevant" and "Relevant" as 1, and "Somewhat Relevant"/"Not Relevant"/"Offensive" as 0.1, in accordance with our previous work\cite{xie2022embedding}. 
% \xiaochen{ruhan: or previously established evaluation framework?}

While this golden dataset with human annotation is of extremely high quality, it can introduce bias in model training, in that all samples come from products occupying top display positions in search, and as a result are much more relevant to the search query than other products not selected in the sample. To ensure that the model is capable of correctly scoring less relevant products, we further expand both the training and the evaluation datasets by including an additional 20\% (query, product) pairs where the query and the product are randomly and independently sampled from all eligible queries and products from the full dataset. These random negative pairs get a score of 0, based on the assumption that on average they are even less relevant than the "Not Relevant" / "Offensive" products that appeared in top search positions. 


% Details regarding the training and evaluation datasets are listed in Table \ref{data}.

% \xiaochen{Xiaochen: More detailed description on how the data are curated will be more than helpful!}

% \xiaochen{Xiao: what are specific details that you'd like to include in the table?}

% \xiaochen{Xiaochen: originally I want to cover the distribution regarding the labels, e.g. how many pairs are labeled as strong relevant? But I find the label of training data are averaged, while for eval data, we do not use soft label before the introduction of random negatives. I am afraid that providing the details regarding label distribution will cause confusion without further explanation why we use different criterion for training/eval datasets.}
\begin{table}[]
\centering
\resizebox{1\columnwidth}{!}{
%\small
\begin{tabular}{ll|lllll}
\hline
                          & & NDCG@5          & NDCG@10         & NDCG@20         & AUROC           \\ \hline
& w/o Negative Sampling      & 89.79          & 90.88          & 92.65          & 91.14          \\
& VNS                        & 90.42          & 91.43          & 93.09          & 94.09          \\
& HNS                        & 90.62          & 91.53          & 93.19          & 90.34          \\ \hline
%& Pseudo Labeler Only  & \textbf{91.58} & \textbf{92.48} & \textbf{93.89} & 93.45          \\
%& Regularization Only & 90.92          & 91.86          & 93.43          & {\underline{95.05}}    \\
\rowcolor{orange!50}
&\CC{}\model               &\CC{}{\textbf{90.96}}    &\CC{}{\textbf{91.91}}    &\CC{}{\textbf{93.47}}    &\CC{}\textbf{95.06} \\ \hline
\end{tabular}
}
\caption{Offline Experiments on Instacart Search Dataset. The highest score is shown in \textbf{boldface}.}
\label{tab:offline}
\end{table}



\subsubsection{Implementation}
\label{sec:offline_implementation}
The present search embedding model serving as the bi-encoder for experiments was originally initialized with a MiniLM-L3-H384-uncased model\footnote{https://huggingface.co/nreimers/MiniLM-L6-H384-uncased} pretrained on paraphrase dataset \footnote{https://www.sbert.net/examples/training/paraphrases/README.html}. It was further finetuned using Instacart's in-house dataset extracted from the search log as described in the reference \cite{xie2022embedding}. The search embedding model is frozen during the training of the cross-encoder model and is only leveraged for guiding negative sampling. 

The cross encoder was initialized with a pretrained MiniLM-L-2-V2 model\footnote{https://huggingface.co/cross-encoder/ms-marco-MiniLM-L-2-v2}. The chunk size of negative sampling is set to 4. The temperature hyperparameter $\tau$ is set to 2 for our method.

% \xiaochen{Taesik: I thought we used the search embedding model as a model checkpoint for the cross encoder, can we double check? cc: Xiao, and Ruhan}

% \xiaochen{Xiaochen: I believe the CE we use is imported from huggingface. We have discussed the idea of using the CE initialized from search embedding model. Unfortunately, it appears that this particular version of the CE became unavailable due to some unexpected issues with your SageMaker instance. And that's why we choose the one available at Huggingface for experiments.}

\subsubsection{Evaluation Metric}

We focus on the two evaluation metrics: Normalized Discounted Cumulative Gain at k (NDCG@k), which measures the effectiveness of the model in a list-wise setting, and Area under the ROC Curve (AUROC), which measures the model's pair-wise performance. For NDCG, we aggregate the data by search queries and evaluate the model's ability to rank the products for each query by their relevance at k = 5, 10, or 20. For AUROC, we convert the classes "Strongly Relevant" and "Relevant" to positive, and the classes "Somewhat Relevant"/"Not Relevant"/"Offensive" as well as the additional random (query, product) pairs to negative, to make the labels binary. 

\subsubsection{Baselines}

We compare our proposed {\modelfull} (BHNS) method with Vanilla Negative Sampling (VNS, Eq.\ref{vanilla}) and Hard Negative Sampling (HNS, Eq.\ref{hard}) strategies as baselines.
% , and further perform ablations on each component of BHNS, i.e., pseduo labeler (Eq. \ref{pseudo}) and sampling regularization (Eq. \ref{reg}) for a deeper investigation. For all methods covered in this experiment, we choose the same models mentioned in Section \ref{sec:offline_implementation} to ensure the consistency. 
Consistent with our experiments on public dataset, we set the chunk size of sampled negatives to 4 for all sampling strategies implemented for fair comparisons. For our method, we set the temperature hyperparameter $\tau$ to 2.

\subsubsection{Result}
\label{sec: offline_results}

 We conduct our experiment as described above and obtain results listed in Table \ref{tab:offline}. The comparison showcases the advantage of adopting false negative sampling strategy, as cross encoder equipped with any negative sampling methods outperform the one without them on nearly all the metrics. Compared to VNS, HNS does not contribute to performance increase in terms of AUROC, and the performance enhancement on NCDG is minimal, implying that the pooling bias introduced during the sampling process impede the thorough exploitation of those informative true hard negatives. As extension, our proposed {\sampler} addresses this shortcoming of HNS by introducing \method, and thus assist cross encoder to manifests more competitive performance.

% The ablation study also underlines the necessity of each component in our proposed BHNS. Merely leveraging pseudo labeler can significantly benefit the model in terms of NDCG, however the lack of any regularization on hard negatives result in unstable AUROC that is slightly lower than the VNS. Only performing regularization on hard negative sampling can enhance the AUROC despite a lower NDCG as the trade off. The combination of these two components achieves a decently improved and balanced performance, showcasing the effectiveness of our bias correction method. 

\subsubsection{Case Study}

To further demonstrate how our {\modelfull} alleviates the pooling bias in the sampling process, we perform intuitive case study to compare {\model} with conventional negative sampling approaches, i.e. VNS and HNS. Given the query \textit{honey}, we retrieve corresponding negative products using VNS, HNS and {\model}, the results are listed in Table \ref{tab:case_study}.

\xiaochen{Taesik: I like the examples. Thank you!}

\xiaochen{Xiaochen: Glad that you enjoy them!}

It is obvious that vanilla negative sampling method is incapable of capturing informative hard negative samples, thus fail to boost the cross encoder via learning from valuable sources. Hard negative sampling strategy, although effectively collecting informative products, assumes the irrelevance between query and sampled products, thus unexpectedly generate the false negatives and introduce the pooling bias. Our method, {\modelfull}, successfully avoids probable false negatives by assigning lower score to them. Also, even though potential false negative products are collected, the pseudo label generation mechanism specially designed to tackle this scenario is able to hint the model about the potential bias, thus achieve the most promising performance.

\begin{table*}[]
\resizebox{1\textwidth}{!}{
\begin{tabular}{lc|lc|lc}
\multicolumn{2}{c|}{VNS}                                          & \multicolumn{2}{c|}{HNS}                                     & \multicolumn{2}{c}{BHNS}                                                   \\ \hline
\textbf{Product Name}                            & \textbf{Label} & \textbf{Product Name}                            & \textbf{Label} & \textbf{Product Name}                                          & \textbf{Label} \\ \hline
bowls, compostable                               & 0              & honey, orange blossom                       & 0              & frozen dairy dessert cookies \& cream                     & 0              \\
potato and wheat chips, cheddar, cheese crispers & 0              & peanuts, honey roasted                      & 0              & dark chocolate, sea salt \& almonds, oat milk, 55\% cocoa & 0              \\
garlic                                           & 0              & moisturizing liquid hand soap milk \& honey & 0              & honey roasted breakfast cereal, whole grain, family size  & 0.019          \\
classic white premium baking chips               & 0              & greek strained yogurt with honey            & 0              & powered donuts pop'ettes                                          & 0        \\\hline
\end{tabular}
}
\caption{Sampled negative products using the query "honey".}
\label{tab:case_study}

\end{table*}


% \begin{table}[]
% \centering
% \resizebox{0.48\textwidth}{!}{
% %\small
% \begin{tabular}{l|l|llll}
% \hline
%                            & & NDCG@5          & NDCG@10         & NDCG@20         & AUROC           \\ \hline
% \multirow{3}{*}{Baselines} & w/o Negative Sampling      & 89.79          & 90.88          & 92.65          & 91.14          \\
% & VNS                        & 90.42          & 91.43          & 93.09          & 94.09          \\
% & HNS                        & 90.62          & 91.53          & 93.19          & 90.34          \\ \hline
% \multirow{3}{*}{Ours} & Pseudo Labeler Only  & \textbf{91.58} & \textbf{92.48} & \textbf{93.89} & 93.45          \\
% & Regularization Only & 90.92          & 91.86          & 93.43          & {\underline{95.05}}    \\
% &\CC{}\model               &\CC{} {\underline{90.96}}    &\CC{} {\underline{91.91}}    &\CC{} {\underline{93.47}}    &\CC{} \textbf{95.06} \\ \hline
% \end{tabular}
% }
% \caption{Offline Experiments on Instacart Search Dataset. The highest score is shown in \textbf{boldface}, while second highest is shown in \underline{underline}. }
% \label{tab:offline}
% \end{table}









% \subsection{A/B Testing}
\subsection{Experiment in Instacart Search}
% To establish the real-world application of {\model}, we conduct online A/B experiment where the cross encoder trained in \ref{instacart_exp} is incorporated into Instacart's search system, and examine its impact on the relevance of search results and user experience. 
\xiaochen{xiao: I tweaked some of the wording in this section, since we are not reporting the results from the a/b test.}

To establish the real-world application of {\model}, we incorporate the cross encoder trained in \ref{instacart_exp} with Instacart's search system, and examine its impact on the relevance of search results. 

\subsubsection{Search System at Instacart}
Search system at Instacart consists of a retrieval stage and a ranking stage. The retrieval stage casts a broad net and retrieves a large number of products related to the search query from multiple sources using both sparse and dense signals. It is followed by a multi-step ranking stage, where ranking models with increasing complexities are applied to filter out less relevant products at each step. This cascade pattern ensures that only high quality search results are presented to the end user. Given the complexity and the latency implication of the cross encoder model, it is tested as part of the final ranking stage, where the top 50 items get reranked to maximize search conversion. 

The final ranker is a LightGBM model \cite{ke2017lightgbm} with a variety of features, such as how relevant the product is to the search query, the product's popularity and availability, user's personal preference, etc. In the baseline ranker model serving in production, the query-product cosine similarity from the existing bi-encoder search embedding model \cite{xie2022embedding} is one of the dominant relevance features. In this experiment, we replace this bi-encoder similarity score with the score from the cross encoder model, and retrain the LightGBM ranker model with the same ranking objective. %The retrained ranker is deployed as a replacement for the existing ranker in the A/B testing, while other components of the search pipeline remain unchanged. 
The retrained ranking is deployed as a replacement for the existing ranker in this test, while other compoments of the search pipeline remain unchanged.

\subsubsection{Evaluation Metric}

In addition to evaluation metrics involved in \ref{tab:offline}, we extend to cover more evaluation metrics, i.e., precision and Mean Reciprocal Rank (MRR) for more comprehensive evaluation.



\subsubsection{Results}
%Before launching the online experiment, we benchmark the performance of the new ranker model against the baseline model on a sample of recent searches from Instacart's business, and compare the two models' performance in ranking, where converted products are taken as positive labels. 

We benchmark the performance of the new ranker model against the baseline model on a sample of recent searches from Instacart's business, and compare the two models' performance in ranking, where converted products are taken as positive labels. The results are listed in Table ~\ref{instacart_offline}. While the other features going into the two ranking models remain identical, replacing the bi-encoder with the cross encoder boosted by {\modelfull} strategy proves to be effective in significantly improving both list-wise and pair-wise ranking metrics. The comparison further demonstrates the superiority of {\modelfull} in handling pooling bias in real-world e-commerce scenario.  

% \begin{table*}[]
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{lllllllll}
% model                     & AUC    & MRR & \shortstack{NDCG\\@5} & \shortstack{NDCG\\@10} & \shortstack{NDCG\\@20} & \shortstack{Precision\\@5} & \shortstack{Precision\\@10} & \shortstack{Precision\\@20} \\ \hline
% ranker w/o CE                  & 89.18                & 57.51               & 76.40  & 79.21 & 80.45   & 20.02      & 12.44  & 8.91      \\
% \rowcolor{orange!50}
% ranker w. CE & \textbf{91.44}               & \textbf{58.73}               & \textbf{77.80}  & \textbf{80.52} & \textbf{81.69} & \textbf{20.46}      & \textbf{12.61}   & \textbf{8.92}   \\
% \hline
% \end{tabular}
% }
% \caption{Offline evaluation on the performance of Instacart's ranking model on search logs. The ranker without cross encoder utilizes relevance score returned by present search embedding model, i.e., bi-encoder, as a relevance feature, which is replaced with the cross encoder score in the experiment.}
% \label{instacart_offline}
% \end{table*}

\begin{table}[]
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{l|l|l}
             & Reranker w/o CE & Reranker w. CE \\ \hline
AUC          & 89.18           & \CC{}\textbf{91.44} \\
MRR          & 57.51           & \CC{}\textbf{58.73} \\
NDCG@5       & 76.40           & \CC{}\textbf{77.80} \\
NDCG@10      & 79.21           & \CC{}\textbf{80.52} \\
NDCG@20      & 80.45           & \CC{}\textbf{81.69} \\
Precision@5  & 20.02           & \CC{}\textbf{20.46} \\
Precision@10 & 12.44           & \CC{}\textbf{12.61} \\
Precision@20 & 8.91            & \CC{}\textbf{8.92}  \\ \hline
\end{tabular}
}
\caption{Evaluation on the performance of Instacart's ranking model on search logs. The ranker without cross encoder utilizes relevance score returned by present search embedding model, i.e., bi-encoder, as a relevance feature, which is replaced with the cross encoder score in the experiment.}
\label{instacart_offline}
\end{table}


% \subsubsection{Deployment}
% The cross encoder is deployed as part of the ranker system, with the model making real-time inference for incoming (query, product) pairs on the fly. An in-memory LRU cache is added to reduce latency and improve system stability, with a cache hit rate of 35\%. 

% \xiaochen{Xiao: the latency increased by 180ms p95. Not sure if we want to mention that? There are ways to further improve latency, from more stable caching to quantization, but we haven't got the time to explore.}

% \xiaochen{Xiaochen: I am not sure if it is a significant increase. Better ask Taesik I think?}

% \subsubsection{Online Results}
% TBD

==> tex/fne.tex <==
\section{Methodology}

To alleviate the pooling bias problem introduced above, we propose a new metric for evaluating the likelihood of false negatives, namely {\method}. Based on this metric, we design our {\modelfull} strategy, depicted in Figure \ref{fig:sampler}.

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{fig/sampler.pdf}
\vspace{-0.1in}
\caption{{\modelfull}. By leveraging {\method}, the sampler detect potential false negatives and function by 1. reducing the weight of potential false negatives during hard negative sampling and 2. informing the model of the likelihood of false negative through pseudo label.}
\label{fig:sampler}
\vspace{-0.1in}
\end{figure*}

\subsection{\method}

Given a query $q_i$ and in-batch off-diagonal product $p_j$, our goal is to estimate the likelihood that $(q_i, p_j)$ is a false negative pair, i.e. the likelihood that $p_j$ is in fact relevant to $q_i$, which is denoted as $E(q_i, p_j)$. Given there is no explicit knowledge regarding the ground truth for the relationship between such in-batch pairs, we turn to estimate this relationship by leveraging Instacart's bi-encoder search embedding model.


We propose the following hypothesis: \textbf{The more similar two queries are, the more likely they share the same relevant product.}

The intuition behind this hypothesis is straightforward. Given the same target product, different users may formulate their search queries differently based on their context \cite{aula2003query}. Since the search embedding model is trained on historical search conversions, it naturally projects these different queries with similar semantic meanings to be close to each other, as well as to the product they converted on, in the semantic space.
% , i.e:

% \begin{equation}
% \label{assump_1}
%     r(q_i, p_j) \rightarrow r(q_j, p_j) \ \ s.t. \text{sim}(q_i, q_j) \rightarrow \max(\text{sim}), i \neq j. 
% \end{equation}



% where $\max(\text{sim})$ denotes the upper bound of similarity metric. 

Similarly, if two queries are semantically independent, then it is likely that their correspondences with the same product are also mutually independent.

% , i.e.:

% \begin{equation}
% \label{assump_2}
%     r(q_i, p_j) \Vbar r(q_j, p_j) \ \ s.t. \text{sim}(q_i, q_j) \rightarrow \min(\text{sim}), i \neq j.
% \end{equation}

% where $\min(\text{sim})$ denotes the lower bound of similarity metric. 
Therefore, we infer that $\text{sim}(q_i, q_j)$ can serve as a measure indicating the extent to which information in $r(q_j, p_j)$ can be transferred to $r(q_i, p_j)$. Based on the inference, we calculate false negative estimation $E(q_i, p_j)$ using $r(q_i, p_j)$ along with $\text{sim}(q_i, q_j)$ as follows:

\begin{equation}
\label{FNE}
   E(q_i, p_j) =  r(q_j, p_j) \cdot \text{sim}(q_i, q_j) \ \ s.t. i \neq j.
\end{equation}

% \xiaochen{Taesik: Should we talk about why $r(q_j, p_j) \cdot \text{sim}(q_i, q_j)$ is better than just $\text{sim}(q_i, p_j)$? I think we can talk about $\text{sim}(q_i, p_j)$ is just an output of the weak learner, while the proposed method uses $r(q_j, p_j)$, a soft label obtained from supervision that can provide more valuable information for training.
% }

% \xiaochen{Xiaochen:Thanks for your suggestion! Will make modification accordingly.
% }

% \xiaochen{Taesik: BTW, $E(q_i, p_j)$ can also be defined as $r(q_i, p_i) \cdot \text{sim}(p_i, p_j)$, have we tried this? or does it make sense we use average value of two values as $E(q_i, p_j)$ ? If we haven't tried this and don't have time to test it, we could simply mention, "One could try this alternative approach, but our proposed methods have proven effective."/
% }

% \xiaochen{Xiaochen: good proposal! Maybe we do not have the time trying the idea for now, but it worth mentioning in some parts of this work.}

where $r(q_j, p_j)$ comes from the training data and already has been labeled, and $\text{sim}(q_i, q_j)$ can be inferred by taking the cosine similarity between the two query embeddings from the bi-encoder search embedding model. The fusion of knowledge derived from the pre-trained bi-encoder and information conveyed through the ground truth labels renders the estimation comprehensive and robust. The computation of $\text{sim}(q_i, q_j)$ can be performed dynamically in the data loading step without introducing significant time-consumption, as it is in the time complexity of $O(n)$.

% When $\text{sim}(q_i, q_j) = 1$, $q_i = q_j$, a false negative will be created according to Eq. \ref{vanilla}; when $\text{sim}(q_i, q_j) = 0$, 

We utilize the estimation of false negative in two ways for optimizing conventional hard negative sampling process (\ref{hard}), i.e., sampling regularization and pseudo label generation, which will be introduced respectively.



% Note that $r(q_i, p_j)$ is gold-standard label existing before the sampling procedure, while $\text{sim}(q_i, q_j)$ can be calculate through the bi-encoder search embedding model. We 


% This assumption is based on previous works focusing on query expansion, where semantically similar queries are generated and 




\subsection{Sampling Regularization}

Compared with vanilla negative sampling (Eq. \ref{vanilla}), hard negative sampling strategy (Eq. \ref{hard}) is even more likely to introduce false negative pairs. To alleviate the problem, we propose to utilize {\method} as an additional regularization term, described as follows:

\begin{multline}
\label{reg}
 \mathbf{r}(q_i, p_j)=0 \ \ \\ s.t. j \in argmax_{k}(\text{sim}(\mathbf{e}_i^q, \mathbf{e}_j^p) \cdot (1-E(q_i, p_j))^\tau), i \neq j.
\end{multline}

where $\tau$ is a temperature hyperparameter curving the weight of $E(q_i, p_j)$. Here, {\method} serves as a regularization term. High $E(q_i, p_j)$ implies that $(q_i, p_j)$ has a high likelihood of being false negative, and Eq. \ref{reg} ensures that the pair has less of a chance to be erroneously selected as a hard negative sample, thus balancing informativeness and robustness and mitigating pooling bias prevalent in conventional hard negative sampling. 




\subsection{Pseudo Label Generation}


While reducing score for potential false negatives diminishes pooling bias, the unsupervised regularization cannot guarantee the extinction of all false negatives. For further eliminating remaining pooling bias caused by these omitted cases, we design dual insurance mechanism as follows:

Instead of indiscriminately assuming off-diagonal query-product pairs $(q_i, p_j)$ are irrelevant as in vanilla negative sampling (Eq. \ref{vanilla}) and hard negative sampling (Eq. \ref{hard}), we adopt {\method} (Eq. \ref{FNE}) to estimate the relevance between $(q_i, p_j)$ that serves as pseudo label for training, i.e.:

% \begin{equation}
% \label{pseudo}
% \mathbf{r}(q_i, p_j)=E(q_i, p_j) \ \ \\ s.t. i \neq j.%, p_j \in \text{sampler}_{k}(\mathcal{P}).
% \end{equation}

% \begin{equation}

\begin{multline}
\label{hard_combined}
         \mathbf{r}(q_i, p_j)=E(q_i, p_j) \ \ \\s.t. j \in argmax_{k}(\text{sim}(\mathbf{e}_i^q, \mathbf{e}_j^p) \cdot (1-E(q_i, p_j))^\tau), i \neq j.
\end{multline}
% \end{equation}


where $\mathbf{r}(q_i, p_j)$ ranges from 0 to $r(q_j, p_j)$, and is proportional to $\text{sim}(q_i, q_j)$. This pseudo label has the following desirable properties: 

\begin{itemize}
\item When $\text{sim}(q_i, q_j)$ equals 1, the two queries $q_i$ and $q_j$ are equivalent, and their relationship with product  $p_j$ is also equivalent, i.e., $\mathbf{r}(q_i, p_j)=r(q_j, p_j)$. 
\item When $\text{sim}(q_i, q_j)$ equals 0, the two queries are independent from each other. Given that the product $p_j$ is relevant to $q_j$, it is highly likely that it is irrelevant to $q_i$, and the pair $(q_i, p_j)$ is unlikely to be a false negative when we set $\mathbf{r}(q_i, p_j)$ to 0. 
\end{itemize}

In this way, the pseudo label generated via {\method} provides an extra correction on the regularized hard negative sampling strategy (Eq. \ref{reg}), further reducing the likelihood of introducing pooling bias in indiscriminate negative labeling. The combination of regularization and pseudo label based on {\method}, namely {\modelfull}, will be evaluated in the next section.


% We can further combine pseudo label generator and sampling regularization to build our {\sampler} as follows:


% % \begin{equation}

% \begin{multline}
% \label{hard_combined}
%          \mathbf{r}(q_i, p_j)=E(q_i, p_j) \ \ \\s.t. j \in argmax_{k}(\text{sim}(\mathbf{e}_i^q, \mathbf{e}_j^p) \cdot (1-E(q_i, p_j))^\tau), i \neq j.
% \end{multline}
% % \end{equation}

==> tex/introduction.tex <==
\section{Introduction}
\label{sec:intro}
In the rapidly evolving landscape of e-commerce search, efficient and accurate inference on product relevance plays a crucial role in enhancing user experiences and driving business success. Transformer-based architectures have been accepted for assessing the relevance between queries and products at Instacart\cite{xie2022embedding}. The training of such sophisticated search relevance models typically necessitates datasets of high quality and ample quantity. However, datasets adopted for training such a model are commonly limited in size and highly imbalanced in the e-commerce scenario. One the one hand, annotating datasets serving for the training are time-consuming and labor-intensive, constraining the volume of labeled data\cite{li2017active}. On the other hand, query-product pairs for annotation are typically pre-collected through basic information retrieval system\cite{cai2022hard, li2017active}. As a result, labeled data are dominated by the relevant pairs, while irrelevant cases are scarce, thus harming the performance of relevance assessment model.

% As users' decision can be swayed by many factors other than relevance, conversion history cannot be directly utilized as golden-standard label on relevance. Human annotated datasets thus serve for the training, however, the time-consuming and labor-intensive nature of manual annotation constrain the volume of labeled data.

% Besides, while relevant query-product pair serve as golden-standard positive cases, high-quality negative cases, which should have been able to help the model to acquire capability of distinguishing irrelevant products from relevant ones, are naturally absent. 

% Unconverted products may not necessarily be irrelevant to the search query, because users' decision can be swayed by many factors other than relevance such as price, size, visual presentation, personal preference for flavor or brand, etc. This is confirmed in our data verification process in examining search logs from Instacart, a leading e-commerce player in on-line grocery shopping, where we found more than 4\% of query-product pairs from the search logs with zero historical conversions are labeled as positive (relevant) by human annotators. 


% In the past, the bi-encoder approach, which independently processes queries and products for similarity calculations, gained widespread acceptance due to its convenience and adaptability. However, the bi-encoder design frequently falls short in capturing the intricate relationships and inherent semantics found within e-commerce data. The interaction between queries and products is merely modeled as a conventional similarity score between embeddings, leading to compromised performance.



% For the performance enhancement, researchers have thoroughly explored the negative sampling strategy, where in-batch products are picked for being combined with query and thus produce query-product pairs labeled as negatives. However, 


% The traditional methods of matching search queries with product listings often fall short in capturing the nuanced relationships and semantics inherent in e-commerce data. 

% To address this challenge, the use of cross encoders has emerged as a promising and innovative approach \cite{Dai_2019}. Cross encoders have gained traction for their ability to model complex interactions between query and product data, serving as reranker and ultimately leading to improved search performance in promoting more relevant products.

% \xiaochen{Taesik: Strictly speaking, "cross encoder" is an architecture-agnostic term that refers to any sequence models which take a pair of query and document as input. I think we can simply remove "a type of transformer-based architecture"}

% \xiaochen{Xiaochen: That makes sense, thanks for your suggestion!}

% For training an advanced model as nuanced as cross encoder, it becomes essential to acquire high-quality data. An important data source for training e-commerce relevance model with decent performance is past search logs with queries and corresponding products that led to conversions. However, while these query-product pair serve as golden-standard positive cases, high-quality negative cases, which should have been able to help the model to acquire capability of distinguishing irrelevant products from relevant ones, are naturally absent. Unconverted products may not necessarily be irrelevant to the search query, because users' decision can be swayed by many factors other than relevance such as price, size, visual presentation, personal preference for flavor or brand, etc. This is confirmed in our data verification process in examining search logs from Instacart, a leading e-commerce player in on-line grocery shopping, where we found more than 4\% of query-product pairs from the search logs with zero historical conversions are labeled as positive (relevant) by human annotators. 

To address the two challenges, researchers at Instacart choose to leverage negative sampling strategy to streamline the training\cite{xie2022embedding}. Negative sampling methods facilitate the generation of irrelevant query-product pairs to complement the positive instances. This approach ensures the provision of a well-balanced training dataset that accurately mirrors the intricacies encountered in real-world e-commerce contexts. It not only aids in augmenting the model's capacity to distinguish relevant from irrelevant query-product pairs but also significantly contributes to the overall resilience and efficacy of the e-commerce search system. 

\begin{figure}[t]
\centering
\includegraphics[width=0.95\columnwidth]{fig/problem.pdf}
\vspace{-0.1in}
\caption{In e-commerce scenario, conventional negative sampling usually assumes the irrelevance between original query and sampled products, which introduces pooling bias by producing false negative pairs such as [Honey, Wildflower Honey] or  [Apple, Apple Sauce]. These samples are wrongly labeled as irrelevant pairs, thus harm the performance of search model.}
\label{fig:problem}
\vspace{-0.1in}
\end{figure}


% While negative sampling strategies effectively mitigate the data insufficiency problem, they introduce another challenge: the emergence of pooling bias during the negative sampling process. 
While negative sampling strategies effectively facilitate the training, they introduce another challenge: the emergence of pooling bias during the negative sampling process. 
In this context, pooling bias refers to the \textbf{utilization of unlabeled positive pairs as false negatives that detrimentally impacts the model's performance\cite{cai2022hard, arabzadeh2022shallow, thakur2021beir}}, as demonstrated in Figure \ref{fig:problem}. 
% In this context, false negatives refer to instances where relevant query-product pairs are mistakenly labeled as irrelevant samples during sampling. 
Conventional negative samplers assume randomly selected query-product pairs to be negative (irrelevant), ignoring the possibility of false negatives. This issue becomes more pronounced for hard negative samplers that explicitly select products with high similarity to the given query, as these query-product pairs have a higher chance of being false negatives without proper control. The presence of false negatives in the training data significantly impacts performance of the search embedding model by introducing noise, potentially leading to overfitting of the model to the true positives and over-penalization of popular products. Therefore, mitigating pooling bias by appropriately addressing false negatives introduced during the sampling process is crucial to ensure that the real-world performance of the models are not compromised.

% \xiaochen{ruhan: nit - confusion--> noise?}
% \xiaochen{Xiaochen: Exactly. Thanks for proposing that and I've made the modification.}

To tackle this problem, in this paper, we present {\method}, a novel method for estimating the probability of query-product pairs being false negatives. We leverage semantic similarity between queries to calculate the false negative likelihood for query-product pairs. We apply the estimation of false negative likelihood to eliminate pooling bias in two ways: 1. guiding the training via generating pseudo labels, and 2. directing the sampling through regularizing the hard negative sampler for enhancement. We combine these two approaches and build our sampling strategy, i.e., {\modelfull} ({\model}). We utilize the proposed {\model} to optimize cross encoder, which takes concatenated query-product pairs as input and serves as advanced relevance assessment model \cite{rendle09bpr, he2017neural}.

For validating the efficacy of our proposed {\model}, we conduct experiments on three settings, i.e., examination on public datasets, offline test with Instacart's in-house data, and A/B testing as part of Instacart's search system. We compare {\model} with conventional negative sampling strategy as well as baselines specifically designed to handle false negative bias to examine the efficacy of {\model}. Through our experimental results and case study, our proposed {\model} demonstrates superior performance, thus provides strong evidence validating the hypotheses underlying {\method} and support the correctness of rationale behind the design of {\model}.

==> tex/related_work.tex <==
\section{Related Work}

\subsection{Cross Encoder for Search}



Compared with typical bi-encoder, cross encoder has demonstrated its more advanced capability in performing ranking\cite{rosa2022defense}. After the emerging of BERT \cite{devlin2018bert}, researchers take a very initial step on ranking with cross encoder by proposing monoBERT \cite{nogueira2019passage}. Researchers further propose to utilize advanced cross encoder for instructing bi-encoder through knowledge distillation \cite{choi2021improving, lin2020distilling, lin2021batch, lu2022ernie,zeng2022curriculum}. Several studies in various domains also propose to combine bi-encoder with cross encoder in a cascade pattern, where the bi-encoder retriever provides informative negatives to facilitate the training of cross encoder serving as ranking\cite{li2021align,lei2022loopitr, zhang2021adversarial}, however, this concept does not function in our application scenario according to our internal experiments.


\subsection{Hard Negative Sampling}

Previous works have thoroughly analyzed the benefit of introducing hard negatives. Comparison between random negative sampling and hard negative sampling demonstrates the effectiveness of heuristical sampling strategy\cite{karpukhin2020dense}. Researchers propose their method to gather global negatives via dense retrieval model \cite{xiong2020approximate}. In the setting of contrastive learning, previous works \cite{robinson2020contrastive, tabassum2022hard} also report that hard negatives are far more informative compared with random negatives, thus induce more competitive performance of models.

While the advantage of exploiting hard negatives has been acknowledged, researchers also notice the problem co-occurring with the sampling procedure. It is discerned that false negatives are introduced through negative sampling process, thus harm the performance of models. Researchers mention that introducing hard negatives indistinguishly might result in performance degradation of bi-encoder architecture, and propose to leverage cross encoder for correcting the bias \cite{qu2020rocketqa}. Adding random negatives along with hard negatives is also proposed as effective solution to alleviate the false negative problem\cite{zhan2021optimizing}. A recent study on recommender system \cite{ma2023exploring} propose to leverage clustering approach to eliminate false negatives and thus obtain so-called "Real Hard Negatives". However, the method is designed to handle sequential information and not suitable to our pair-wise ranking scenario. Model leveraging similarity between positive and negative cases to estimate the probability of false negative is also proposed in the domain of computer vision\cite{zhang2022false}. Study in the domain of knowledge graph also proposes that labels generated by clustering algorithm is capable of guiding model to avert false negatives\cite{je2022entity}. Similarly, supervised models replying on data augmentation and is utilized for identifying potential false negative\cite{huynh2022boosting}. However, these methods require the availability of trainable embedding of entity, whose implementations are unfeasible while cross encoder is applied. It is also proposed that the introduction of an additional IPW-based risk model can eliminate the false negative \cite{cai2022hard}, while its simultaneous training of two cross encoder pattern will introduce considerable additional time consumption. 

As the conclusion of this section, most of previous works focus on false negative problem in the setting of bi-encoder, while researches on cross encoder regarding negative sampling are rare due to the lack of independent embedding of query/product that can guide the heuristic sampling process. 
